Demonstration of PI2: Interactive Visualization Interface Generation for SQL Analysis in Notebook

We demonstrate PI2, the first notebook extension that can automatically generate interactive visualization interfaces during SQL-based analyses.

==> implementation.tex <==
\section{Design}
\subsubsection{Query Selection}
In order to generate interfaces, Precision Interfaces requires an input query log. The interface generation extension allows a user to select individual code cells containing SQL queries to include as part of the input query log to a generated interface. When the user clicks the "Generate Interface" toolbar button, the selected queries are retrieved from the notebook, combined into a query log, and sent to the Precision Interfaces back end for processing.

\subsubsection{Generated Interface Panel}


\subsubsection{Versioning}
As the user presses the "Generate Interface" button over the course of an analysis, the extension tracks different generated interface versions. Each successive generated interface is assigned a version number (e.g. "V1", "V2", ...). Versions are displayed as tabs in the Generated Interfaces Panel, allowing the user to revisit old interfaces.

A user returning to an interface version some time after initially generating it may not remember how the interface was generated. It is important that the results in a notebook are reproducible, and knowing what code generates a particular result is a fundamental part of reproducibility.

However, since we use a side-by-side panel design, the user does not have the context of a code cell above the generated result. Furthermore, the input queries to the interface may be messily dispersed across the entire notebook (identified in \cite{Head2019ManagingMI} as one of the primary sources of "messes" in notebooks). Code cells are also mutable, meaning that the code used to generate an interface may no longer be present in the notebook. As such, indicating which input code cells were included in the query log of an interface is a poor choice for conveying how an interface is generated.

To remedy this, the interface generation extension saves the input query log when the interface is generated and surfaces the log as a sub-section (collapsed by default) of the Generated Interface Panel. If a user wishes to see what queries generated a given interface, they can expand the input query log section.

\subsubsection{Export}

Once a user has generated an interface and begun interacting with it to visualize data, they may want to use what they're currently looking at in the Generated Interface Panel as part of some further work in the context of the notebook. To this end, the interface generation extension provides an "export" button which will append a new code cell to the notebook containing the current query specified by the interface configuration. This enables a workflow in which the user authors queries, generates an interface to work with the parameters of those queries in a more interactive context, and returns to the notebook context with new code.

\subsection{Implementation}

We implement the proposed interface generation design as a Jupyter Lab extension. Jupyter Lab \cite{jupyterlab} is an interactive development environment first released in 2018 that provides a side-by-side interface for viewing and editing Jupyter notebooks. It includes an extension system which allows users to augment the Jupyter Lab interface with additional functionality in the form of menus, panels, buttons, commands, and more. The Jupyter Lab extension API also includes provisions that allow extensions to inject new UI as React components, modify the contents of notebooks, and persist state.

The Precision Interfaces back end operates purely on query logs and emits interface specifications. It can be thought of as a function $f(\text{Query log}) \rightarrow \text{UI specification}$. However, this computation is expensive, taking multiple seconds as it searches a large space of possible difftrees, so we choose to run it as a network service and issue interface generation requests to it over the network from the notebook extension code. After the user selects queries and presses the "Generate" button, the extension serializes the selected queries into a query log and issues an HTTP request to the Precision Interfaces server. The response comes in the form of a JSON interface specification, which is then rendered in the Generated Interfaces panel as a new interface version.

The database, too, is accessed over the network. As the user reconfigures the query by interacting with the interface, the extension issues queries against the database and updates the visualizations.

Once an interface is generated, the input query log, Difftree, and initial widget configuration are stored as a new version in the extension's state and surfaced to the user as a new tab in the Generated Interfaces Panel. The latest widget configuration is persisted to the extension state so that the user can return to a notebook later and see the last configuration and corresponding visualization.

\subsection{Limitations}

Precision Interfaces is designed to be language-agnostic. However, it currently only supports SQL, so our integration is limited to the use case of SQL-based data analysis in notebooks.

We assume that the database schema is immutable. If the database schema were to be changed by a SQL code cell, queries in prior cells would no longer be valid. Since generated interfaces generate queries based on the syntax of the input queries, this would also make older versions of generated interfaces stop working. As such, we are limited to evaluating interfaces generated for data analysis workflows that exclusively issue SELECT queries and do not change the data set in-place. Even with this limitation, there is still a wide breadth of queries that can be expressed due to Precision Interfaces' ability to generate interfaces for arbitrary query logs.

==> system.tex <==
\section{Interface Generation}\label{s:details}
\vspace{-2mm}
\begin{figure}[h]
  \centering
  \includegraphics[width=\columnwidth]{figure/pipeline.pdf}
  \vspace{-7mm}
  \caption{\sys interface generation pipeline.}
  \vspace{-4mm}
  \label{f:pipeline}
\end{figure}

\sys transforms an input sequence of queries into an interactive interface in four steps (\Cref{f:pipeline}).
\textcircled{1} It first parses the input query sequence $Q$ into \difftrees. 
\textcircled{2} \sys maps the \difftrees
to an interface.
An interface mapping $\mathbb{I}=(\mathbb{V},\mathbb{M},\mathbb{L})$ is defined by a mapping $\mathbb{V}$ from \difftrees to visualizations, a mapping $\mathbb{M}$ from choice nodes to interactions,
and a layout mapping $\mathbb{L}$. We formulate the interface mapping problem as a schema matching problem by defining schema for both \difftree and interfaces. 
\textcircled{3} A cost model $C(\mathbb{I}, Q)$ evaluates the interface and \sys either returns the interface or  
chooses a valid transformation to apply to the \difftrees.  
Informally, our problem is to return the lowest cost interface $\mathbb{I}$ that can express all queries in $Q$.
\textcircled{4} The space of possible interfaces is enormous, so we solve this problem using Monte Carlo Tree Search~\cite{Coulom2006EfficientSA}. In this section, we discuss each component in \sys with the example in \Cref{f:difftree}.

\begin{figure}[t]
  \centering
  \includegraphics[width=0.9\columnwidth]{figure/transform.pdf}
  \vspace{-3mm}
  \caption{(a) Three shortened input queries. (b) Initial \difftree for 3 queries and its interface. (c) \difftree Transformation and the interface for transformed \difftree. Node Schemas are annotated in \aqua{Cyan}.}
  \vspace{-5mm}
  \label{f:difftree}
\end{figure}

\subsection{\difftree and Transformation}
\subsubsection{\difftree}

Each query is modeled as its abstract syntax tree (AST). 
A \difftree $\Delta$ compactly represents a set of queries using {\it Choice Nodes}--\texttt{ANY}, \texttt{MULTI}, and \texttt{SUBSET} to encode syntactic differences between queries. Each choice node denotes a subtree in which two or more query ASTs differ. {\tt ANY} chooses one of its children with {\tt} OPT as its special case when there is a single child.  {\tt MULTI} repeats its children mutiple times and {\tt SUBSET} represents the subset of its children. For example, the \difftree in \Cref{f:difftree}(b) encodes the three queries in \Cref{f:difftree}(a) via an {\tt ANY} node. 





\stitle{Result Schema.} 
We define a \difftree's result schema to further determine its visualization mapping.  
By construction, all ASTs' result schemas in a \difftree must be union compatible, namely, the type\footnote{\sys support three types: {\tt num}, {\tt str} and {\tt AST}.} must be the same. The \difftree's result schema is the union of all ASTs' result schemas. For example, the \difftree in \Cref{f:difftree}(b) expresses three queries with their result schema as {\small{\tt <p:\\num,count:num>}}, {\small{\tt <p:num,count:num>}}, and {\small{\tt <a:num,count:num>}}, respectively. Thus, this \difftree's result schema is {\small{\tt <num,num>}}. 

\stitle{Node Schema.}
All choice nodes and their ancestors---collectively, {\it dynamic nodes}---are annotated with node schemas that describe the structural variation expressible by the subtree rooted at the node.
The node schema is a list of expressions over types and node schemas where the operators are $\texttt{|, ?, *}$.  The operator \texttt{|} is the \textit{or} relation 
(\texttt{ANY}), \texttt{?} is the \textit{existential} relation (\texttt{OPT}, \texttt{SUBSET}), and \texttt{*} is \textit{repetition} (\texttt{MULTI}). For example, the {\tt ANY} in \Cref{f:difftree}(b) is varying the child AST, so its node schema is {\small{\tt <AST|AST|AST>}}, i.e. {\small {\tt <AST>}} for short. The other {\tt ANY} in \Cref{f:difftree}(c) is varying numbers, thus its node schema is {\small{\tt <num>}}. 

\subsubsection{\difftree Transformation}
We define a set of \difftree transformation rules that are guaranteed to preserve or increase the expressiveness of the \difftrees.

\stitle {Initial \difftree. } \sys takes all the input queries' ASTs and partition them based on the union compatibility of {\textit result schema}. All the ASTs in one partition will merge into a \difftree with a single {\tt ANY} as its root node. For instance, the three queries in \Cref{f:difftree}(a) have union compatible result schemas so they are in one partition. \Cref{f:difftree}(b) shows the initial \difftree of these queries.

\stitle{Transformation.} 
After applying three transformation rules – {\tt Cluster}(Cluster $Q_{1,2}$), {\tt Split}(split the {\tt ANY} into two \difftrees), {\tt Pushdown}(push down the {\tt ANY} node), this initial \difftree can be transformed into a \difftree shown in \Cref{f:difftree}(c) where the left \difftree has an {\tt ANY} expressing the query differences in {\tt Q1, Q2}.  

\subsection{The Interface Mapping Problem}
A candidate interface $\mathbb{I}=(\mathbb{V},\mathbb{M},\mathbb{L})$ consists of visualization ($\mathbb{V}$), interaction ($\mathbb{M}$), and layout ($\mathbb{L}$) mappings. We model the interface mapping problem as a schema matching problem between matching source (\difftree, choice node) and target (visualization and interaction). Finally, we assign the layout $\mathbb{L}$.

\subsubsection{Visualization Mapping $\mathbb{V}$.}
Each visualization encodes data attributes using a set of visual variables~\cite{bertin1983semiology} (e.g., x and y positions, size, color) and enforces constraints over the data types mapped to those visual variables, e.g. x and y in Bar chart can only be Categorical and Quantitative.
In \Cref{f:difftree}(b), the result schema is {\small {\tt <num, num>}} and with the catelog information that {\tt p} and {\tt a} have low cardinality, we can infer the first {\tt num} type can be treated as Categorical. Thus, such a result schema is able to map to Bar chart. 

\subsubsection{Interaction Mapping $\mathbb{M}$.}

One of the major challenges is to ensure that the interface contains sufficient interactions (both widget and visualization interactions) for the user to interactively express the input queries (and perhaps others).  
\sys manages a library of interaction templates, and identifies candidate interaction mappings for a given choice node\footnote{Technically, \sys maps dynamic nodes (choice node or an ancestor) to interactions, but we focus on choice nodes for clarity as the principles are the same. } based on schema matching. 

\stitle{Widget.}
A widget $w(D)$ is initialized with a choice node's domain $D$ and it can be mapped to a choice node based on its node schema. For instance, a list of buttons can choose a single option and is thus compatible with \texttt{ANY}, a toggle is compatible with \texttt{OPT}, etc.  
For example, the {\tt ANY} node in \Cref{f:difftree}(b) has its schema as {\tt<AST>} which varies 3 ASTs. A button list shown in the right interface can be a candidate, i.e. when clicking on {\tt Q1} buttons, the {\tt Q1} result will update in the visualization. Similarly, a radio list can also be a candidate.

\stitle{Visualization Interaction.}
A visualization can support multiple interactions that help specify the option of choice nodes.  For example, Bar chart supports brush, click, Multi-Click.  In \Cref{f:difftree}(c), the {\tt ANY} node schema is {\small {\tt <num>}} encoding the number difference. By checking the schemas and constraints, click on the right upper visualization can generate such variation too. Thus, in \cref{f:difftree}(c), clicking the bar in the upper visualization will specify {\tt a} value in the \difftrees and further updates the lower visualization. 


\subsubsection{ Layout Mapping ~$\mathbb{L}$.}

After visualization and interaction mapping, we construct a layout tree where leaf nodes are visualizations or widgets, and map inner nodes to horizontal (\texttt{H}) or vertical (\texttt{V}).  Thus, we derive a candidate $\mathbb{L}$. In \Cref{f:difftree}, the layout tree is a vertical node connecting the visualization and buttons. 

 \subsection{Monte Carlo Tree Search}
Same queries can be expressed by different \difftree structures via tree transformations. Each \difftree can have multiple interface mappings. To find the best interface, this subsection introduces a cost model to quantify the goodness of interfaces followed by the  problem formulation and our solution of Monte Carlo Tree Search.  

\subsubsection{Cost Model $C(\mathbb{I}, Q)$.}
$C(\mathbb{I}, Q)$ takes an interface's usability and layout into account. 
For usability, we borrow the equations from SUPPLE~\cite{gajos2004supple}, which models the time to manipulate and navigate between interactions.
For layout, if the interface size exceeds the desired maximum, we add a penalization. 

\begin{problem}[Interface Generation Problem] \label{p:problem}
  Given input query sequence $Q$ and cost model $C(\mathbb{I}, Q)$, return an interface mapping $\mathbb{I}^*=(\mathbb{V},\mathbb{M},\mathbb{L})$ such that $\mathbb{I}$ expresses $Q$ and minimizes $C(\mathbb{I}, Q)$.
\end{problem}

\subsubsection{Monte Carlo Tree Search}
Each set of \difftrees is a state, and transformation rules define the transitions. Since the number of applicable transformation rules is very large, we adopt Monte Carlo Tree Search~\cite{Coulom2006EfficientSA} (MCTS) which employs the UCT strategy to select the next search state that balance the simulated cost and visit time. 
To quickly assess the quality of each state during MCTS, we apply the cost model to $K$ random interface mappings and assign the lowest cost to this state.
Finally, MCTS returns a set of \difftrees, and we perform a complete search for the final interface mapping $\mathbb{I}$.




